Dynamic Diffusion Transformer

Diffusion Transformer (DiT), an emerging diffusion model for image generation, has demonstrated superior performance but suffers from substantial computational costs. Our investigations reveal that these costs stem from the static inference paradigm, which inevitably introduces redundant computation in certain diffusion timesteps and spatial regions. To address this inefficiency, we propose Dynamic Diffusion Transformer (DyDiT), an architecture that dynamically adjusts its computation along both timestep and spatial dimensions during generation. Specifically, we introduce a Timestep-wise Dynamic Width (TDW) approach that adapts model width conditioned on the generation timesteps. In addition, we design a Spatial-wise Dynamic Token (SDT) strategy to avoid redundant computation at unnecessary spatial locations. Extensive experiments on various datasets and different-sized models verify the superiority of DyDiT. Notably, with <3% additional fine-tuning iterations, our method reduces the FLOPs of DiT-XL by 51%, accelerates generation by 1.73, and achieves a competitive FID score of 2.07 on ImageNet. The code is publicly available at https://github.com/NUS-HPC-AI-Lab/ Dynamic-Diffusion-Transformer.

==> sec/deprecated_3_method.tex <==
\section{Dynamic Diffusion Transformer}
\vspace{-2mm}
% In Section~\ref{sec:predliminary}, we introduce diffusion models and the Diffusion Transformer (DiT) \citep{peebles2023scalable}. Subsequently, we present our proposed timestep dynamic width (TDW) approach and spatial-wise dynamic token (SDT) strategy in Sections~\ref{sec:dynamic_channel} and \ref{sec:dynamic_token}, respectively. Finally, Section~\ref{sec:training} outlines the training process of our method.
% ⭕️
In Section~\ref{sec:predliminary}, we provide an overview of diffusion models and the Diffusion Transformer (DiT) \citep{peebles2023scalable}. Next, we introduce the proposed timestep-wise dynamic width (TDW) approach and spatial-wise dynamic token (SDT) strategy of our DyDiT in Sections~\ref{sec:dynamic_channel} and \ref{sec:dynamic_token}, respectively. Finally, Section~\ref{sec:training} details the training process of our method.

\vspace{-3mm}
\subsection{Preliminary} \label{sec:predliminary}
\vspace{-3mm}
\paragraph{Diffusion Models.}
Diffusion models \citep{ho2020denoising, song2020score, nichol2021improved, rombach2022high} generate images from random noise through a series of diffusion steps. These models typically consist of a forward diffusion process and a reverse denoising process. In the forward process, given an image $\mathbf{x}_0 \sim q(\mathbf{x})$ sampled from the data distribution, Gaussian noise $\epsilon \sim \mathcal{N}(0, I)$ is progressively added over $T$ steps. This process is defined as $q\left(\mathbf{x}_t \mid \mathbf{x}_{t-1}\right)=\mathcal{N}\left(\mathbf{x}_t ; \sqrt{1-\beta_t} \mathbf{x}_{t-1}, \beta_t \mathbf{I}\right)$, where $t$ and $\beta_t$ denote the timestep and noise schedule, respectively. In the reverse process, the model removes the noise and reconstructs the image $\mathbf{x}_0$ from the noisy sample $\mathbf{x}_T \sim \mathcal{N}(0, I)$ using $p_\theta\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t\right)=\mathcal{N}\left(\mathbf{x}_{t-1} ; \mu_\theta\left(\mathbf{x}_t, t\right), \Sigma_\theta\left(\mathbf{x}_t, t\right)\right)$, where $\mu_\theta\left(\mathbf{x}_t, t\right)$ and $\Sigma_\theta(\mathbf{x}_t, t)$ represent the mean and variance of the Gaussian distribution.

% Diffusion models \citep{ho2020denoising, song2020score, nichol2021improved, rombach2022high} can generate an image from random noises using a series of diffusion steps. They typically contain a sampling process and a reverse process. In the sampling process, given an image $\mathbf{x}_0 \sim q(\mathbf{x})$ sampled from the dataset distribution, Gaussian noise $\epsilon \sim \mathcal{N}(0, I)$ is gradually added to it in $T$ steps. It can be formulated as $q\left(\mathbf{x}_t \mid \mathbf{x}_{t-1}\right)=\mathcal{N}\left(\mathbf{x}_t ; \sqrt{1-\beta_t} \mathbf{x}_{t-1}, \beta_t \mathbf{I}\right)$, where t and $\beta_t$ denote the timestep and the noise schedule, respectively. The reverse process progressively removes noise and restores image $\mathbf{x}_0$ from Gaussian distribution $\mathbf{x}_{T} \sim \mathcal{N}(0, I)$: $p_\theta\left(\mathbf{x}_{t-1} \mid \mathbf{x}_t\right)=\mathcal{N}\left(\mathbf{x}_{t-1} ; \mu_\theta\left(\mathbf{x}_t, t\right), \Sigma_\theta\left(\mathbf{x}_t, t\right)\right)$, where $\mu_\theta\left(\mathbf{x}_t, t\right)$ and $\Sigma_\theta(\mathbf{x}_t, t)$ denote the mean and variance of a Gaussian distribution. 
% The former should be learned by a neural network, while the latter can be set to $\beta_t \mathbf{I}$ or obtained by learning. 
% ⭕️

% \vspace{-3mm}
% \paragraph{Diffusion Transformer} (DiT) \citep{peebles2023scalable} exhibits scalability properties and promising performance \citep{videoworldsimulators2024}. Similar to \cite{dosovitskiy2020image, vaswani2017attention}, DiT comprises a stack of layers containing a multi-head self-attention block (MHSA) and a multi-layer perception (MLP) block, which can be expressed as $\mathbf{X} \leftarrow \mathbf{X} + \alpha \text{MHSA}(\gamma \mathbf{X} + \beta), \mathbf{X} \leftarrow  \mathbf{X}  + \alpha^{\prime} \text{MLP}(\gamma^{\prime} \mathbf{X} + \beta^\prime)$ where $\mathbf{X} \in \mathbb{R}^{N \times C}$ denotes image tokens. $N$ and $C$ represent the token number and channel dimension, respectively.  The parameters $\{\alpha, \gamma,\beta, \alpha^{\prime}, \gamma^{\prime}, \beta^{\prime} \}$ are obtained from an adaptive layer norm (adaLN) block \citep{perez2018film}, which takes class condition embedding $\mathbf{E}_{cls}$ and timestep embedding $\mathbf{E}_t$ as input.  Given an input $\mathbf{x}_t$ at the $t$-th timestep,  DiT is trained to estimate $\mu_\theta\left(\mathbf{x}_t, t\right)$ mentioned above via a noise prediction task, supervised by $\mathcal{L}_{\text{simple}}=\left\|\epsilon_\theta\left(\mathbf{x}_t\right)-\epsilon_t\right\|^2$. To enhance performance, an additional variational lower bound loss $\mathcal{L}_{\text{VLB}}$  is included to optimize $\Sigma_\theta(\mathbf{x}_t, t)$. Therefore, total loss in DiT can be formulated as $\mathcal{L}_{\text{DiT}} = \mathcal{L}_{\text{simple}} + \mathcal{L}_{\text{VLB}}$.

\paragraph{Diffusion Transformer} (DiT) \citep{peebles2023scalable} exhibits the scalability and promising performance of Transformers \citep{videoworldsimulators2024}. Similar to ViT \citep{dosovitskiy2020image}, DiT consists of layers composed of a multi-head self-attention (MHSA) block and a multi-layer perceptron (MLP) block, described as $\mathbf{X} \leftarrow \mathbf{X} + \alpha \text{MHSA}(\gamma \mathbf{X} + \beta), \mathbf{X} \leftarrow  \mathbf{X}  + \alpha^{\prime} \text{MLP}(\gamma^{\prime} \mathbf{X} + \beta^\prime)$, where $\mathbf{X} \in \mathbb{R}^{N \times C}$ denotes image tokens. Here, $N$ is the number of tokens, and $C$ is the channel dimension. The parameters $\{\alpha, \gamma,\beta, \alpha^{\prime}, \gamma^{\prime}, \beta^{\prime} \}$ are produced by an adaptive layer norm (adaLN) block \citep{perez2018film}, which takes the class condition embedding $\mathbf{E}_{cls}$ and timestep embedding $\mathbf{E}_t$ as input
% At each time step, DiT 
% At timestep $t$, given input $\mathbf{x}_t$, DiT is trained to estimate $\mu_\theta\left(\mathbf{x}_t, t\right)$ via a noise prediction task, supervised by the loss $\mathcal{L}_{\text{simple}}=\left\|\epsilon_\theta\left(\mathbf{x}_t\right)-\epsilon_t\right\|^2$. To further improve performance, a variational lower bound loss $\mathcal{L}_{\text{VLB}}$ is included to optimize $\Sigma_\theta(\mathbf{x}_t, t)$. Thus, the total loss in DiT is defined as $\mathcal{L}_{\text{DiT}} = \mathcal{L}_{\text{simple}} + \mathcal{L}_{\text{VLB}}$.



% ⭕️
% For brevity, we omit the layer norm \citep{ba2016layer} before MHSA and MLP. 
% ⭕️
% (adaLN) block \citep{perez2018film, karras2019style, dhariwal2021diffusion}




\vspace{-2mm}
\subsection{Timestep-wise Dynamic Width} \label{sec:dynamic_channel}
\vspace{-2mm}
As mentioned before, DiT spends equal computation for different timesteps, although not all steps share the same generation difficulty (\figurename~\ref{fig:figure1}(a)). Therefore, the \emph{static} computation paradigm introduces significant redundancy in those ``easy'' timesteps. Inspired by structural pruning methods~\citep{he2017channel, hou2020dynabert, fang2024structural}, we propose a \emph{timestep-wise dynamic width} (\textbf{TDW}) mechanism, which adjusts the width of DiT in different timesteps. Note that TDW is not a pruning method that permanently removes certain model components, but rather remains the full capacity of a DiT and dynamically activates different heads/channel groups in each timestep.



% treats each timestep equally and adopts a static architecture to process input $\mathbf{x}_t$. Using uniform computational resources for all timesteps can lead to redundant computation and reduced efficiency during generation. This encourages us to explore a \textit{dynamic} architecture at different timesteps.  Structure pruning methods \eg \citep{he2017channel, hou2020dynabert, fang2024structural} have proven that reducing the model width is an effective way to reduce the computation. Inspired by this insight and the observation in Figure~\ref{fig:figure1} (a), we propose the timestep-wise dynamic width (TDW) method, which adjusts the width of DiT at different timesteps.
% ⭕️

\vspace{-2mm}
\paragraph{Heads and channel groups.} Given input $\mathbf{X}\!\in\!\mathbb{R}^{N \times C}$, an MHSA block employs three linear layers (Q, K, and V) with weights $\mathbf{W}_{\text{Q}}, \mathbf{W}_{\text{K}}, \mathbf{W}_{\text{V}}\!\in\!\mathbb{R}^{C \times (H \times C_H)}$ to project it into query, key, and value tokens, respectively. Here, $H$ denotes the head number and $C=\!\!H\!\times\!C_H$. An output projection is performed using another linear layer (O) with $\mathbf{W}_{\text{O}}  \in \mathbb{R}^{(H \times C_H) \times C}$ weight. Thus, the operation of MSHA can be expressed as
$\text{MSHA}(\mathbf{X}) = \sum_{h=0}^{H} \mathbf{X}_{\text{attn}}^{h} \mathbf{W}_{\text{O}}^{h,:, :} = \sum_{h=0}^{H} (\operatorname{Softmax}((\mathbf{X}\mathbf{W}_{\text{Q}}^{:,h,:}) (\mathbf{X}\mathbf{W}_{\text{K}}^{:,h,:})^{\top}) \mathbf{X} \mathbf{W}_{\text{V}}^{:, h, :}) \mathbf{W}_{\text{O}}^{h,:, :}$.


% Before introducing how to dynamically adjust the width, we first introduce the definition of head in MHSA blocks and channel group in MLP blocks, respectively. The organization of heads and channel groups are presented in Figure~\ref{fig:main} (a, left).
% We first introduce the definition of head in MHSA blocks and channel group in MLP blocks, respectively.
% The organization of heads and channel groups are presented in Figure~\ref{fig:main} (a, left).


% Our goal is to devise a strategy for dynamically adjusting the number of heads used in each timestep, rather than consistently employing all $H$ heads.


% Based on the insight that different timesteps might require different inference costs (\figurename~\ref{fig:figure1}(a)), our goal is to devise a strategy for dynamically adjusting the number of heads used in each timestep, rather than consistently employing all $H$ heads.
% ⭕️



In an MLP block, there are two linear layers with weights $\mathbf{W}_{1} \in \mathbb{R}^{C \times D}$ and $\mathbf{W}_{2} \in \mathbb{R}^{D \times C}$, where $D$ represents the hidden channels. For convenience, we divide $D$ hidden channels into $H$ channel groups, each containing $D_{H} = D / H$ channels, where $H \ll D$.  This operation helps us to reduce the parameters of routers, which will be introduced in the following. Hence, the weight can be reformulated into $\mathbf{W}_{1} \in \mathbb{R}^{C \times (H \times D_{H})}$ and $\mathbf{W}_{2} \in \mathbb{R}^{(H \times D_{H}) \times C}$. Then, the operation in MLP can be formulated as $\text{MLP}(\mathbf{X}) = \sum_{h=0}^{H}\sigma(\mathbf{X}_{\text{hidden}})\mathbf{W}_{2}^{h,:,:} = \sum_{h=0}^{H}\sigma(\mathbf{X} \mathbf{W}_{1}^{:, h, :})\mathbf{W}_{2}^{h,:,:}$. 



Our goal is to develop a strategy to dynamically change the number of activated heads and channel groups in MHSA and MLP blocks during generation. 

% Similar to MHSA, we also need to develop a strategy to dynamically change the number of channel groups used in the MLP across different timesteps. 
% ⭕️


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/main.pdf}
\vspace{-6mm}
\caption{\textbf{Overview of the proposed dynamic diffusion transformer (DyDiT)}. It reduces the computational redundancy in DiT \citep{peebles2023scalable} from both timestep and spatial dimensions. For brevity, we omit the layer norm \citep{ba2016layer} and adaLN~\citep{perez2018film} blocks in DiT.} 
\vspace{-6mm}
\label{fig:main}
\end{figure*} 












\vspace{-2mm}
\paragraph{Head and channel activation based on timestep.}
We first take the activation of heads in an MHSA block as an example. Given the timestep embedding $\mathbf{E}_t \in \mathbb{R}^{C}$ within the DiT, we feed it into a linear router layer $\mathbf{W}_{\text{head}} \in \mathbb{R}^{C \times H}$ followed by a sigmoid function, resulting in a set of probabilities $\mathbf{R}_{\text{head}} = \{r^1, r^2...r^h...r^H\} \in \mathbb{R}^{H}$, where $r^h$ denotes that the probability of $h$-th head to be activated. We adopt a threshold of 0.5 to convert it into a binary mask $\mathbf{M}_{\text{head}}$ to indicate the activation results of heads. $\mathbf{M}_{\text{head}}^{h} =1$ indicate the $h$-th head is selected to activate otherwise $\mathbf{M}_{\text{head}}^{h} =0$ means that it should be deactivated. Regarding the MLP block, another router layer $\mathbf{W}_{\text{channel}} \in \mathbb{R}^{C \times H}$ is employed to predict the probability of keeping each channel group $\mathbf{R}_{\text{channel}}$. Similar to the head activation, we obtain a mask $\mathbf{M}_{\text{channel}}$ indicating whether to activate this channel. Benefiting from the grouping operation in hidden channels, there are only $C\times H$ rather than $C\times D_{H}$ parameters in a router, reducing parameters number obviously since $H \ll D_{H}$. Note that the parameters of routers are NOT shared among transformer layers. %Figure~\ref{fig:main} (a) provides a visualization of TDW.  % ⭕️


\vspace{-2mm}
\paragraph{Training.}
During training, we directly apply the mask to the corresponding featuremap ($\mathbf{X}_{\text{attn}}$ or $\mathbf{X}_{\text{hidden}}$) to zero out the deactivated heads or channel groups. This is achieve through $\text{MSHA}(\mathbf{X}) = \sum_{h=0}^{H} \mathbf{M}_{\text{head}}^h \cdot \mathbf{X}_{\text{attn}}^{h} \mathbf{W}_{\text{O}}^{h,:, :}$ and $\text{MLP}(\mathbf{X}) = \sum_{h=0}^{H}\mathbf{M}_{\text{channel}}^h \cdot \sigma(\mathbf{X}_{\text{hidden}})\mathbf{W}_{2}^{h,:,:}$, where $\cdot$ denotes the Hadamard product. To address the non-differentiability of the threshold operation, we employ the straight-through-estimator \citep{bengio2013estimating} during back-propogation.  This approach utilizes the gradient of $\mathbf{M}_{\text{head}}$ and $\mathbf{M}_{\text{channel}}$ as the gradient for $\mathbf{R}_{\text{head}}$ and $\mathbf{R}_{\text{channel}}$, respectively, enabling the end-to-end training of TWD.
 % ⭕️

\paragraph{Inference.}
During inference, we can pre-determine the activated heads and channel group offline at each timestep, slimming the weights $\{\mathbf{W_{\text{Q}}},\mathbf{W_{\text{K}}}, \mathbf{W_{\text{V}}}, \mathbf{W_{\text{O}}} \}$ in MHSA blocks and $\{ \mathbf{W}_1, \mathbf{W}_2 \}$ in MLP blocks. This reduces the computational cost associated with deactivated heads and channel groups at each timestep. The right part of Figure~\ref{fig:main} (a)  provides a visualization of the TDW. 
 % ⭕️









\vspace{-2mm}
\subsection{Spatial-wise Dynamic Token} \label{sec:dynamic_token}
\vspace{-2mm}
In addition to computational redundancy across different timesteps, as shown in Figure~\ref{fig:figure1}(b), redundancy in the spatial dimension arises from varying difficulty levels in noise prediction for image patches. To address this, we propose a spatial-wise dynamic token (SDT) method to reduce computational costs for patches where noise estimation is straightforward.
 % ⭕️


\vspace{-2mm}
\paragraph{Bypassing the MLP block.}
DyDiT adaptively identifies the tokens associated with image regions that present lower noise prediction difficulty and allows these tokens to bypass the computationally intensive MLP blocks to reduce the redundant computation. Note that theoretically, this block-skipping operation can be applied to both MHSA and MLP blocks. However, the MHSA block is crucial for conducting token interactions, which we find essential for generation. Skipping MHSA block may result in a loss of important information and negatively impact performance~\citep{chen2024pixart}. More critically, varying numbers of tokens bypassing across images during generation can result in incomplete tensor shapes, 
prohibiting batched inference and reducing generation throughput. Therefore, we apply this operation only in the MLP block for each transformer layer in DiT.
 % ⭕️

 
\vspace{-2mm}
\paragraph{Training.}
To identify the tokens to bypass an MLP block, we feed the input tokens $\mathbf{X}\!\in\!\mathbb{R}^{N \times C}$ into a router layer $\mathbf{W}_{\text{token}} \in \mathbb{R}^{C \times 1}$, followed by a sigmoid function to predict the probability $\mathbf{R}_{\text{token}} \in \mathbb{R}^{N}$. We then convert it into a binary mask $\mathbf{M}_{\text{token}}$ using a threshold of 0.5. Each element $\mathbf{M}^{i}_{\text{token}}$ in the mask indicates whether the $i$-th token should be processed by the block  (if $\mathbf{M}_{\text{Token}}^{i} =1$) or directly bypassed (if $\mathbf{M}_{\text{Token}}^{i} =0$). Notably, the router parameters are not shared across transformer layers. During training, similar to TDW, we perform the Hadamard product between the obtained mask $\mathbf{M}_{\text{token}}$ and the output of MLP to to incorporate the router  $\mathbf{W}_{\text{token}}$ within the gradient flow via $ \mathbf{M}_{\text{token}} \cdot \text{MLP}(\mathbf{X})$. Employing the straight-through-estimator \citep{bengio2013estimating},  we utilize the gradient of $\mathbf{M}_{\text{token}}$ to approximate the gradient of $\mathbf{R}_{\text{token}}$, facilitating end-to-end training of spatial-wise dynamic token strategy.
 % ⭕️


\vspace{-2mm}
\paragraph{Inference.}
During inference, we directly apply the mask $\mathbf{M}_{\text{token}}$ to gather those tokens for input into the MLP, thereby avoiding unnecessary computational costs for other tokens. Then, we adopt a scatter operation to reposition the processed tokens according to $\mathbf{M}_{\text{token}}$. We present this in Figure~\ref{fig:main} (b). Since there is no token interaction within the MLP, the SDT operation supports batched inference, improving the practical generation efficiency. 
 % ⭕️






\subsection{Dynamic Model Training} \label{sec:training}
\vspace{-2mm}
Given a pre-trained DiT model, we fine-tune it on the target dataset using our proposed methods, resulting in the dynamic model, DyDiT. We demonstrate how to control the FLOPs budget of DyDiT and stabilize the training process.
 % ⭕️
 
\vspace{-2mm}
\paragraph{Training with FLOPs-constrained loss.}
We design a FLOPs-constrained loss to control the computational cost during the generation process. We find it impractical to obtain the entire computation graph during $T$ timesteps since the total timestep $T$ is large \eg $T=1000$. Fortunately, during the DiT training, the timesteps in batch data are sampled from $t \sim \text{Uniform}(0, T)$, which approximately covers the entire computation graph. Assuming each training batch contains $B$ samples, with $t_b$ as the timestep for the $b$-th sample, we compute the total FLOPs at the sampled timestep, $P^{t_b}$, using masks $\{ \mathbf{M}_{\text{head}}^{t_b}, {\mathbf{M}}_{\text{channel}}^{t_b}, \mathbf{M}_{\text{token}}^{t_b} \}$ from each transformer layer, as detailed in Section~\ref{sec:dynamic_channel} and Section~\ref{sec:dynamic_token}.  Let $P_{\text{total}}$ denote the total FLOPs of MHSA and MLP blocks in the original DiT. We formulate the FLOPs-constrained loss as $\mathcal{L}_\text{FLOPs} = (\frac{1}{B}\sum_{t_b} \frac{P^{t_b}}{P_{\text{total}}} - \lambda)^2
$, where $\lambda$ represents the budget FLOPs ratio, and each $t_b$ is uniformly sampled from the interval [0, T]. The overall training objective combines this FLOPs-constrained loss with the original DiT training loss, expressed as $
\mathcal{L}_\text{total} = \mathcal{L}_\text{DiT} + \mathcal{L}_\text{FLOPs}
$. During training, the gradient flow can propagate backward through the masks $\{ \mathbf{M}_{\text{head}}^{t_b}, {\mathbf{M}}_{\text{channel}}^{t_b}, \mathbf{M}_{\text{token}}^{t_b} \}$ to optimize routers in TDW and SDT. 
 % ⭕️

\vspace{-2mm}
\paragraph{Stabilizing training.}
In practice, we find directly fine-tuning DyDiT with $\mathcal{L}_\text{total}$ might lead to unstable training. To address this, we employ two techniques to stabilize training. First, alongside training with $\mathcal{L}_\text{total}$, we maintain a complete DiT model supervised by the same target as the dynamic model, introducing an additional loss, $\mathcal{L}_{\text{DiT}}^{\text{complete}}$, for a warm-up phase. After this phase, we remove the complete model's loss and continue training solely with $\mathcal{L}_\text{total}$. Additionally, prior to fine-tuning, we rank the heads and hidden channels in MHSA and MLP blocks based on a magnitude criterion~\citep{he2017channel}. We consistently select the most important head and channel group in TDW. This ensures that at least one head and channel group is activated in each MHSA and MLP block across all layers and timesteps, thereby avoiding instability caused by dropping an entire block.
 % ⭕️


% Different from models for visual perception tasks like image classification, diffusion model is more hard to training \eg requiring more training iterations.







% Hence, we propose a dynamic token selection method to reduce the computational cost on those patches that easy to estimate the noise. 
% Specifically, before a block, it selects some tokens and inputs them into the block, while other tokens directly bypass the block. 
% However, since $\operatorname{MHSA}$ is adopted to conduct interaction between tokens, some tokens bypass this block obviously hurts the performance and results in incomplete tensor shape, prohibiting the batch inference. Hence, we adopt conduct this before $\operatorname{MLP}$ block.
% During inference, we directly apply the mask $\mathbf{M}_{\text{MLP}}^{\text{token}}$ to gather those tokens that need to be input into $\operatorname{MLP}$, avoiding the computational cost for other tokens. 

% Each element of it $\mathbf{M}^{i} =1$ denotes that $i$-th token will be processed by the block, while $\mathbf{M}^{i} =0$ represents the token will directly bypass the block. 

% This can be formulated as $  \frac{\partial \mathcal{L}}{\partial \mathbf{\pi} } \approx \frac{\partial \mathcal{L}}{\partial \mathbf{M} } $
% The obtained mask $M$ is element-wisely product with the output of $\operatorname{MLP}$ to



% we also add Gumbel Noise \cite{jang2016categorical} into the Softmax function to enable stochastic training.




% to enable the end-to-end training.


% \paragraph{Inference paradigm.}
% During inference, we can pre-determined the weights in both the MHSA and $\operatorname{MLP}$ blocks to reduce the computational cost on dropped heads and channels in the current timestep. The right part of Figure~\ref{fig:main} (a)  provides a visualization of the TDW. Since the selection of width is solely based on the timestep embedding $\mathbf{E}_t$, the architecture at each timestep can be pre-determined offline, avoiding additional cost during inference.


% \paragraph{Self-distillation via the complete model}
% Since the complete architecture of DiT is still available in the dynamic process, we propose a self-distillation method to leverage this good property. Specifically, given the model with parameters $\theta$, it performs predictions based on the dynamic architecture learned from TDW and SDT. Let $F_{\theta}(\mathbf{x}_t)$ denotes its prediction and $\mathcal{L}_\text{DiT}$ represents the associated loss. Additionally, the same parameters can be used for predictions using the complete architecture, dented as $F_{\theta}^{\text{Teacher}}$. Since this complete architecture employs more parameters during estimation, we assume it achieves better accuracy and thus designates it as the teacher for the dynamic architecture. We adopt $\mathcal{L}_\text{DiT}^{\text{Teacher}}$ to denote its prediction loss. Consequently, the distillation loss can be formulated as
% $\mathcal{L}_\text{Distill} = \left\|F_{\theta}(\mathbf{x}_t)-F_{\theta}^{\text{Teacher}}(\mathbf{x}_t)\right\|^2$.
% ⭕️

% The model can also conduct prediction with the same parameters but the complete architecture through $F_{\theta}^{\text{teacher}}(\mathbf{x}_t)$.
% Since more parameters are employed during estimation, we assume that it has better estimation accuracy and adopt it as the teacher of dynamic architecture. 


% We adopt $\mathcal{L}_\text{DiT}^{\text{teacher}}(\mathbf{x}_t)$ to denote its prediction loss.



% In the following, we will first introduce the preliminary knowledge of diffusion models and Diffusion Transformer (DiT) \citep{peebles2023scalable} in Section~\ref{sec:predliminary}. Subsequently, we present the proposed temporal-wise dynamic width approach and spatial-wise dynamic token strategy in Section~\ref{sec:dynamic_channel} and Section~\ref{sec:dynamic_token}, respectively.
% Finally, we discuss the training objectives and inference paradigm in Section~\ref{sec:complete}. 



% \begin{equation}
% \mathbf{X} \leftarrow \mathbf{X} + \alpha \operatorname{MHSA}(\gamma \mathbf{X} + \beta), 
% \end{equation}
% \begin{equation}
% \mathbf{X} \leftarrow  \mathbf{X}  + \alpha^{\prime} \operatorname{MLP}(\gamma^{\prime} \mathbf{X} + \beta^\prime),
% \end{equation}

% \paragraph{Head/Channel importance ranking.}
% Instead of directly managing to adjust channels, we first measure the importance of heads in $\operatorname{MHSA}$ and channels $\operatorname{MLP}$. Like pruning method \citep{molchanov2016pruning}, we adopt the variation of the loss when a head or channel is removed as the importance score of the head.  We accumulate the importance score across total $T$ timesteps. Thus, the importance score of a head in an $\operatorname{MHSA}$ block can be expressed as $S_{\text{Attn}}^{h} = \sum_{t=0}^{T} \left|\frac{\partial \mathcal{L}_{\text{DiT}}^{t}}{\partial \mathbf{X}_{\text{Attn}}^{h,t}} \mathbf{X}_{\text{Attn}}^{h,t} \right|$, where $\mathbf{X}_{\text{Attn}}^{h,t}$ denotes the feature of head $h$ at the $t$-th timestep.
% Unlike $\operatorname{MHSA}$, we can measure the importance for each channel $d$ in hidden space $D$. This can be formulated as$
% S_{\text{Hidden}}^{d} = \sum_{t=0}^{T} \left| \frac{\partial \mathcal{L}_{\text{DiT}}^{t}}{\partial \mathbf{X}_{\text{Hidden}}^{d, t} } \mathbf{X}_{\text{Hidden}}^{d, t}   \right |$.
% Note that the importance score is also aggregated across $N$ tokens, although we omit this detail from the above equations for clarity.  A high importance score indicates that a head or channel significantly influences the noise prediction. Once we obtain these scores, we reorder them by adjusting the weights within $\operatorname{MHSA}$ and $\operatorname{MLP}$ in descending order of importance, as depicted in Figure~\ref{fig:main} (a).
% ⭕️ 
% Differently, since there are total $T$ timesteps in the diffusion model,
% \begin{equation}
% S_{MLP}^{d} = \sum_{t=0}^{T} \sum_{c=0}^{C} \left| \frac{\partial \mathcal{L}_{DiT}^{t}}{\partial \mathbf{W}_{1}^{c, d} }  +  \frac{\partial \mathcal{L}_{DiT}^{t}}{\partial \mathbf{W}_{2}^{d, c} }   \right |
% \end{equation}

%In each layer of the transformer, we adopt this method to reduce computational redundancy

% To handle the non-differentiable threshold operation, following the straight-through-estimator \cite{bengio2013estimating}, we adopt the gradient of $\mathbf{M}_{\text{Head}}$ and $\mathbf{M}_{\text{Channel}}$ as the gradient of $K_{\text{Head}}$ and $K_{\text{Channel}}$ during back-propogation, respectively.


% During inference, we can pre-determined the weights in both the MHSA and $\operatorname{MLP}$ blocks to reduce the computational cost on dropped heads and channels in the current timestep. The right part of Figure~\ref{fig:main} (a)  provides a visualization of the TDW. Since the selection of width is solely based on the timestep embedding $\mathbf{E}_t$, the architecture at each timestep can be pre-determined offline, avoiding additional cost during inference.



% \vspace{-3mm}
% \paragraph{Advantage.}
% The design of the temporal-wise dynamic width offers two advantages. First, because the dynamic strategy relies solely on the timestep information, the architecture can be pre-determined offline, incurring no additional cost during inference.  Furthermore, this method supports batch inference without requiring any mask operations during inference, thus avoiding the most common issues encountered in existing dynamic networks \cite{yin2021adavit, zhao2024dynamic}. % ⭕️




% Thus, it can be seamlessly combined with existing efficient diffusion methods to achieve better efficiency.
% Furthermore, different from some dynamic neural networks \eg \cite{yin2021adavit}, which is hard to achieve actual acceleration on GPUs due to many mask operations.


==> sec/deprecated_4_experiment.tex <==
\vspace{-3mm}
\section{Experiments}
\vspace{-3mm}
\paragraph{Implementation details.}
We conduct experiments based on diffusion transformer (DiT) \citep{peebles2023scalable} by default. We fine-tune a pre-trained DiT model on a target dataset to enable dynamic architecture learning. We adopt three DiT models with different sizes, denoted as DiT-S/B/XL. All models are pre-trained on ImageNet \citep{deng2009imagenet} with a resolution of 256$\times$256. For DiT-XL, we directly adopt the checkpoint from the official DiT repository \footnote{https://github.com/facebookresearch/DiT}, while for DiT-S and DiT-B, we leverage pre-trained models \footnote{https://github.com/NVlabs/T-Stitch} provided by \citet{pan2024t}. All models are with a patch size of 2. Details of DiT models are presented in our Appendix~\ref{app:details}. To maintain consistency with DiT, we set the learning rate to 1e-4 and the global batch size to 256. All experiments are conducted on a server with 8$\times$NVIDIA A800 80G GPUs. The strength of classifier-free guidance is set to 1.5 and 4.0 for evaluation and visualization, respectively. Following DiT,  we use 250 DDPM \citep{ho2020denoising} sampling steps, unless otherwise specified. For the fair comparison with DiT, we sample 50,000 images to measure the Fréchet Inception Distance (FID) \citep{heusel2017gans} score and adopt the ADM’s TensorFlow evaluation suite \citep{dhariwal2021diffusion} to conduct the evaluation. We measure the generation speed on an NVIDIA V100 32G GPU. % ⭕️ 



\vspace{-4mm}
\paragraph{Datasets.}
Apart from ImageNet  \citep{deng2009imagenet}, to comprehensively evaluate our method, we also report the performance and efficiency on four fine-grained datasets used in \citet{xie2023difffit}, including Food \citep{bossard2014food}, Artbench \citep{liao2022artbench}, Cars \citep{gebru2017fine} and Birds \citep{wah2011caltech} in in-domain fine-tuning and cross-domain transfer learning manners. Images in these datasets are also resized into 256$\times$256 resolution.  % ⭕️







% \paragraph{Evaluation Metrics.}
% Following prior works, we sample 50,000 images to measure the Fréchet Inception Distance (FID) \citep{heusel2017gans} score. We adopt the ADM’s TensorFlow evaluation suite \citep{dhariwal2021diffusion} to conduct the evaluation.  % ⭕️



% Inception Score (IS) \citep{salimans2016improved}, sFID \citep{nash2021generating}, and Prevision-Recall \citep{kynkaanniemi2019improved} are also reported for complementary.




\vspace{-3mm}
\subsection{Comparison with Pruning Methods}
\vspace{-3mm}
\paragraph{Benchmark}
Efficient diffusion methods have predominantly focused on U-Net \citep{ronneberger2015u} architectures in prior research . However, the exploration of efficient diffusion transformers \citep{peebles2023scalable} remains an unaddressed area. Since the proposed temporal-wise dynamic width and spatial-wise dynamic token improves the model efficiency from structure and token perspective, respectively, they are closely related to structure pruning and token pruning methods. To comprehensively evaluate the superiority of our approach, we establish a benchmark across diverse datasets and compare our methods against representative structure and token pruning techniques. To facilitate the comparison, all experiments in this section are conducted based on DiT-S. % ⭕️




Random pruning, Magnitude pruning \citep{herrmann2020channel}, and Taylor pruning \citep{molchanov2016pruning} are three effective structure pruning methods designed for perception tasks and also demonstrate effectiveness on diffusion models with U-Net architecture \citep{fang2024structural}. We adopt different pruning criteria from them to distinguish important heads and channels in DiT from from less significant ones. We also include diff-pruning \citep{fang2024structural} in the comparison, which is a Taylor-based pruning method specifically optimized for the diffusion process. We directly drop 50\% least important heads and channels. % ⭕️


We also compare our methods with a training-free token pruning technique, ToMe \citep{bolya2022token}, which progressively prunes tokens in each vision transformer \citep{dosovitskiy2020image} layer through token merging. Its enhanced version \citep{bolya2023token} can also accelerate diffusion models based on U-Net architectures \eg Stable Diffusion \citep{rombach2022high} .  We directly apply the enhanced version in each layer of DiT. % ⭕️



\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/flops/DiT-S_flops_fid.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/flops/DiT-S_flops_fid.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/flops/DiT-S_flops_fid.pdf}
    \end{subfigure}
    \caption{FLOPs-FID}
    \label{fig:my_main_figure}
\end{figure}




% Since previous model-based efficient diffusion methods are mainly designed for U-Net \citep{ronneberger2015u} architecture, the exploration of efficient diffusion transformers is still absent. The proposed timestep-based width selection (TWS) and dynamic token selection (DTS) improve the efficiency from the structure-level and token-level, which are highly related to structure pruning and token pruning methods, respectively. To comprehensively evaluate the superiority of our method, we build a benchmark across diverse datasets and compare our methods with representative structure and token pruning methods. 




\vspace{-3mm}
\paragraph{In-domain fine-tuning on fine-trained datasets.}
We first compare our methods with structure pruning and token pruning methods on fine-grained datasets. The experimental details are presented in Appendix~\ref{app:exp_fine}. Results are summarized in Table~\ref{tab:sota_finegrained}. With the pre-defined FLOPs ratio $\lambda$ set to 0.5, our methods can remarkably reduce the computational cost and enhance the generation speed while maintaining performance levels comparable to the original DiT. 
Notably, our approach even surpasses the original DiT on the Car and Bird datasets, owing to the well-learned strategy to adjust the architecture. To ensure fair comparisons, we set pruning ratios to 50\% for other pruning methods aiming for similar FLOPs. Among structure pruning techniques, Magnitude pruning exhibits relatively better performance, yet our method consistently outperforms it by a substantial margin. Although ToMe \citep{bolya2023token} demonstrates success in accelerating U-Net models with minimal performance loss, applying it to DiT leads to performance degradation. Since DiT lacks convolutional layers, the error introduced by ToMe’s token merging operation becomes irrecoverable even with subsequent training. This means that ToMe is not suitable to accelerate the diffusion transformer. % ⭕️

% The performance of Structure pruning methods varies on different datasets and Magnitude pruning achieves relative better performance. 
% However, our method still outperform it by a large margin. 
% When it comes to the token pruning method, although ToMe \citep{bolya2023token} can accelerate models based on U-Net with small performance loss, applying it into DiT results in performance collapsed.
% Since there are not any convolutional layers in DiT, the error introduced by token merging operation from ToMe is hard to recover even  with training. This means that ToMe not suitable to accelerate the diffusion transformer.




\begin{table}[t]
\normalsize
\addtolength{\tabcolsep}{0.5mm}
\renewcommand{\arraystretch}{0.8}
    \centering
    \caption{\textbf{Comparison with pruning methods on fine-grained datasets.} We sample 50,000 images and leverage FID to measure the generation quality. }
\resizebox{1.0\textwidth}{!}{    \begin{tabular}{c | c | c |c c c  c }
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{s/img $\downarrow$ } & \multirow{2}{*}{FLOPs (G) $\downarrow$}  & \multicolumn{4}{c}{FID $\downarrow$} \\
    & &
    & \multicolumn{1}{c}{Food}  & \multicolumn{1}{c}{Artbench}  & \multicolumn{1}{c}{Car}   & \multicolumn{1}{c}{Bird}   \\ \midrule

    Original DiT-S  &  0.65 & 6.07  & \textbf{14.56} & \textbf{17.54} & \underline{11.52} & \underline{11.62}  \\
    From Scratch  & \textbf{0.38}  & \underline{3.05}   & 67.24 & 82.78 & 66.55 & 108.83  \\  \midrule

    
    \multicolumn{7}{c}{\emph{Structure Pruning Methods}} \\

    Random pruning & \textbf{0.38} & \underline{3.05}   & 76.69 & 102.65 & 116.30 & 76.69  \\
    Magnitude Pruning   & \textbf{0.38} & \underline{3.05} & 42.04  & 52.96   & 37.21 & 26.46  \\
    Taylor Pruning & \textbf{0.38}  & \underline{3.05}  & 95.97 & 104.94 & 57.22 & 95.22 \\
    Diff Pruning & \textbf{0.38}  &\underline{3.05}   & 81.47 & 128.09 & 99.41 & 89.59  \\ \midrule

    \multicolumn{7}{c}{\emph{Token Pruning Methods}} \\
    ToMe $r=50\%$  & 0.43  & \textbf{2.95}   & 288.56 & 271.53 & 316.68 & 297.70   \\
    ToMe $r=50\%$ w/ training & 0.43  & \textbf{2.95}   & 241.79 & 235.84 & 291.41 & 197.50   \\
    ToMe $r=20\%$ & 0.61  & 4.82   & 147.57 & 163.17 & 221.97 & 158.57  \\   

    ToMe $r=5\%$ & - & -   & - & - & - & -  \\   
    \midrule
    
\multicolumn{7}{c}{\emph{The proposed Dynamic Diffusion Transformer}}\\
    DyDiT-S $\lambda=0.5$ & \underline{0.42}  & 3.08    & \underline{14.73} & \underline{21.75} & \textbf{11.49} & \textbf{8.96}  \\     \bottomrule
    \end{tabular}}
    \label{tab:sota_finegrained}
     \vspace{-3mm}
\end{table}






\begin{table*}[!h]
\renewcommand{\arraystretch}{0.8}
      \begin{minipage}{0.49\linewidth}
    \caption{\textbf{Comparison with pruning methods on ImageNet \citep{deng2009imagenet}.} We sample 50,000 images and leverage FID to measure the generation quality. }
 
        \centering
        \small

\resizebox{1.0\textwidth}{!}{    \begin{tabular}{c | c  c c}
    \toprule
    \multirow{1}{*}{Method} & \multirow{1}{*}{s/img $\downarrow$ } & \multirow{1}{*}{FLOPs (G) $\downarrow$}   & \multicolumn{1}{c}{FID $\downarrow$}     \\ \midrule

    Original DiT-S  & 0.65  & 6.07  & \textbf{21.46}   \\
    From Scratch  & \textbf{0.38}  & 3.05   & 92.36  \\  \midrule

    
    \multicolumn{4}{c}{\emph{Structure Pruning Methods}} \\

    Random pruning & \textbf{0.38}   & 3.05 & 64.45  \\
    Magnitude Pruning  & \textbf{0.38}   & 3.05   & 53.18  \\
    Taylor Pruning   & \textbf{0.38}   & 3.05    & 59.46 \\
    Diff Pruning   & \textbf{0.38}   & 3.05  & 55.88   \\ \midrule

    \multicolumn{3}{c}{\emph{Token Pruning Methods}} \\
    ToMe  $r=50\%$  & 0.43  & \textbf{2.95}  & 262.20 \\
    ToMe  $r=50\%$ w/ training & 0.43  & \textbf{2.95}   & 214.09   \\
    ToMe  $r=20\%$ & 0.61  & 4.82     & 139.33   \\  
    ToMe $r=5\%$    & - & - & -   \\   
    \midrule
    
\multicolumn{4}{c}{\emph{The proposed Dynamic Diffusion Transformer}}\\

    DyDiT-S $\lambda=0.5$  & \underline{0.42}  & \underline{2.97}  & \underline{31.83} \\     \bottomrule

    \end{tabular}}
   \label{tab:sota_imagenet}
    \end{minipage}
    \hfill %前后不要有空格
    \begin{minipage}{0.49\linewidth}
          \caption{\textbf{Scale up the model size.} $\lambda$ is set to 0.5 for all DyDiT models.``FID $\Delta \downarrow$'' denotes the FID gap between our DyDiT and its DiT counterpart. With the increasing model size, the performance gap narrows. The largest model DyDiT-XL even outperforms DiT-XL, while introducing much less computational cost.}  % ⭕️
 
        \centering
        \small
        %\resizebox{\linewidth}{!}{
\resizebox{0.95\textwidth}{!}{\begin{tabular}{c | c | c | c| c}
\toprule
    \multirow{1}{*}{Model} & \multirow{1}{*}{s/img $\downarrow$ } & \multirow{1}{*}{FLOPs (G) $\downarrow$}  & \multicolumn{1}{c|}{FID $\downarrow$}   & \multicolumn{1}{c}{FID $\Delta \downarrow$}  \\ \midrule

    DiT-S  & 0.65  & 6.07   & 21.46 & +0.00 \\
    DyDiT-S & 0.42 & 2.97 & 31.83  & +10.37 \\  \midrule

    DiT-B  &  2.09  & 23.02   & 9.07 & +0 \\
    DyDiT-B &  1.26 & 11.68 &  14.89 & +5.82 \\  \midrule

    DiT-XL  &   10.22 &  118.69  & 2.27  & +0.00 \\
    DyDiT-XL &  6.47 &  68.41    & 2.14  & -0.13 \\      \bottomrule
 

    \end{tabular}}
        %}
        \label{tab:size}
    \end{minipage}
     \vspace{-5mm}
\end{table*}







% Compared with structure pruning methods, the performance drop of our methods is more marginal. 








% the performance of both our method and structure pruning methods drops obviously due to the decrease of computation during sampling. 

\begin{table}[t]
\normalsize
\addtolength{\tabcolsep}{0.5mm}
\renewcommand{\arraystretch}{0.8}
    \centering
    \caption{\textbf{Experiments of cross-domain transfer learning.} ``Original DiT-S'' denotes directly fine-tuning DiT on downstream datasets. Our proposed methods aim to simultaneously learn the dynamic architecture and perform domain transfer during the fine-tuning process.} % ⭕️
\resizebox{0.8 \textwidth}{!}{    \begin{tabular}{c | c | c |c c c  c }
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{s/img $\downarrow$ } & \multirow{2}{*}{FLOPs (G) $\downarrow$}  & \multicolumn{4}{c}{FID $\downarrow$} \\
    & &
    & \multicolumn{1}{c}{Food}  & \multicolumn{1}{c}{Artbench}  & \multicolumn{1}{c}{Car}   & \multicolumn{1}{c}{Bird}   \\ \midrule
    Original DiT-S  &  0.65 & 6.07  & \underline{14.56} & \underline{17.54} & \textbf{11.52} & \underline{11.62}  \\ \midrule

    DyDiT-S $\lambda=0.3$ &  \textbf{0.32}  & \textbf{2.12}    & 60.05  & 59.12 & 89.59 & 55.26 \\  
    DyDiT-S $\lambda=0.5$ & \underline{0.42}  & \underline{3.13}    &  16.64 & 26.08 & 21.01 & 20.26  \\    
    DyDiT-S $\lambda=0.7$ & 0.53  & 4.52   & 17.02 & 20.85 & 16.14 & \textbf{11.37} \\    
    DyDiT-S $\lambda=0.8$ & 0.60  & 5.10   & \textbf{13.38} & \textbf{17.52} & \underline{12.42} & 12.03 \\     \bottomrule
    \end{tabular}}
    \label{tab:cross_domain}
    \vspace{-5mm}
\end{table}










% \begin{table}[t]
% \normalsize
% \addtolength{\tabcolsep}{0.5mm}
% \renewcommand{\arraystretch}{0.8}
%     \centering
%     \caption{\textbf{Comparison with pruning methods on ImageNet \citep{deng2009imagenet}.} We sample 50,000 images and leverage FID to measure the generation quality. }
% \resizebox{1.0\textwidth}{!}{    \begin{tabular}{c | c | c |c c c  c c}
%     \toprule
%     \multirow{1}{*}{Method} & \multirow{1}{*}{s/img $\downarrow$ } & \multirow{1}{*}{FLOPs (G) $\downarrow$}  & \multicolumn{1}{c}{IS $\uparrow$}  & \multicolumn{1}{c}{FID $\downarrow$}  & \multicolumn{1}{c}{sFID $\downarrow$}   & \multicolumn{1}{c}{Precision $\uparrow$} & \multicolumn{1}{c}{Recall $\uparrow$}     \\ \midrule

%     Original DiT-S  & 0.65  & 6.07   & \textbf{70.93} & \textbf{21.46} & \textbf{7.17} & \textbf{0.63} & \underline{0.56}  \\
%     From Scratch  & \textbf{0.38}  & 3.05   & 14.41 & 92.36 & 19.06 & 0.26 & 0.34  \\  \midrule

    
%     \multicolumn{8}{c}{\emph{Structure Pruning Methods}} \\

%     Random pruning & \textbf{0.38}   & 3.05  & 23.91 & 64.45 & 15.02 & 0.37 & 0.48  \\
%     Magnitude Pruning \citep{he2017channel}  & \textbf{0.38}   & 3.05  & 28.88 & 53.18 & 11.11 & 0.44 & 0.53  \\
%     Taylor Pruning \citep{molchanov2016pruning}  & \textbf{0.38}   & 3.05   & 26.65 & 59.46 & 15.19 & 0.40 & 0.51  \\
%     Diff Pruning \citep{fang2024structural}  & \textbf{0.38}   & 3.05  & 28.06 & 55.88 & 12.88 & 0.42 & 0.52  \\ \midrule

%     \multicolumn{8}{c}{\emph{Token Pruning Methods}} \\
%     ToMe \citep{bolya2023token} $r=50\%$  & 0.43  & \textbf{2.95}  & 2.34 & 262.20 & 175.24 & 0.10 & 0.00  \\
%     ToMe \citep{bolya2023token} $r=50\%$ w/ training & 0.43  & \textbf{2.95} & 5.14  & 214.09   & 133.16 & 0.07 & 0.12   \\
%     ToMe \citep{bolya2023token} $r=20\%$ & 0.61  & 4.82    & 8.02 & 139.33 & 88.48 & 0.21 & 0.30  \\     \midrule
    
% \multicolumn{8}{c}{\emph{The proposed Dynamic Diffusion Transformer}}\\

%     DyDiT-S $\lambda=0.5$  & \underline{0.42}  & \underline{2.97}  & \underline{50.54} & \underline{31.83} & \underline{9.73} & \underline{0.56} & \textbf{0.59} \\     \bottomrule

%     \end{tabular}}
%     \label{tab:sota_imagenet}
% \end{table}


\subsection{Experiments on ImageNet}
\vspace{-3mm}
\paragraph{Comparison with pruning methods on ImageNet.}
To further compare the performance of our method and pruning methods, we conduct experiments on ImageNet \citep{deng2009imagenet}. All methods are initialized from the pre-trained DiT model and then fine-tuned on ImageNet to adapt the pruned or dynamic architecture.  More experimental details can be found in Appendix~\ref{app:exp_imagenet}. From Table~\ref{tab:sota_imagenet}, both our proposed method and pruning approaches exhibit performance degradation due to reduced computation during sampling. However, the impact on our method is comparatively marginal. The performance decline of our method can be attributed to the intricate distribution present in ImageNet, necessitating a model with sufficient capacity. Further reducing the computation of the original DiT-S, which has only 6.07 GFLOPs, prevents DyDiT-S from achieving this capacity.  This motivates us to investigate model size scaling in the subsequent section.  % ⭕️

% Unlike the fine-grained datasets discussed earlier, ImageNet poses greater complexity. 

\vspace{-3mm}
\paragraph{Scale up the model size.}
Based on the observation from DyDiT-S and DiT-S, we assume that the model should have sufficient capacity to handle the complex data distribution in challenging datasets like ImageNet and believe that the performance gap between DyDiT and DiT will diminish as the model size increases. To verify this, we fine-tune DiT-B and DiT-XL with the proposed methods for 100,000 and 150,000 iterations, obtaining DyDiT-B and DyDiT-XL, respectively. We provide additional details regarding the model configurations in Appendix~\ref{app:model_size}. The results are summarized in Table~\ref{tab:size}.  As we scale the model size from ``S'' to ``B'', the FID score gap between DyDiT-B and DiT-B narrows. Notably, at the largest model size (``XL''), our model DyDiT-XL even achieves a slightly better FID score while utilizing only 57\% of the computational cost and 63\% of the generation time compared to DiT. These results validate the scalability potential of our approach. % ⭕️


% To verify this, we conduct experiments on DiT-B and DiT-XL, which are fine-tuned on ImageNet by 100,000 and 150,000 iterations, respectively. 
% Based on the experiments on DiT-S, we find that the proposed method can obviously improve the efficiency while maintaining the performance on those fine-grained datasets, since the distribution of these datasets are relatively simple. But when it comes to ImageNet, the performance of DiT-S also drops obviously. We attribute this phenomenon to that the distribution of ImageNet is complex, and the model should have enough computation to fit. 
% The size of DiT-S is already small, further reducing its computation leads to unavoidable performance drop. 





% We consider a more challenging scenario, where the model need to learn the dynamic str
\vspace{-3mm}
\subsection{Cross-domain transfer learning}
\vspace{-3mm}
Transferring a pre-trained model to downstream datasets is a common practice to leverage existing diffusion models. In our experiments, we aim to validate the effectiveness of this method in a scenario that is often overlooked by existing pruning techniques. Specifically, we consider a DiT model pre-trained on ImageNet and investigate its ability to simultaneously learn dynamic architecture and transfer to downstream fine-grained datasets. More details are presented in Appendix~\ref{app:exp_cross}.  We summarize the results in Table~\ref{tab:cross_domain}. Compared with the in-domain fine-tuning (as shown in Table~\ref{tab:sota_finegrained}), DyDiT requires a larger ratio $\lambda$ (\eg 0.7 and 0.8) to achieve comparable performance with the original DiT, due to the challenging nature of the cross-domain transfer. Although the superiority of DyDiT is not as significant as that of in-domain fine-tuning, it still offers accelerated generation speed. We hope that future research will consider incorporating our methods for cross-domain transfer learning. % ⭕️















% \begin{table*}[!h]
% \renewcommand{\arraystretch}{0.8}

%  \begin{minipage}{0.49\linewidth}

%      \caption{\textbf{Ablation studies based on DyDiT-S.} ``TWS'': Time-based width selection. ``DTS'': Dynamic token selection. ``CMT'': Complete model teacher.} % ⭕️
%           \label{tab:ablation_study}
%   \centering
%   \small
%   %\resizebox{\linewidth}{!}{
% \resizebox{1.0 \textwidth}{!}{    \begin{tabular}{c | c c c |c c c }
%    \toprule 
%     \multirow{2}{*}{Model} & \multirow{2}{*}{TWS} & \multirow{2}{*}{DTS} & \multirow{2}{*}{CMT}  & \multicolumn{3}{c}{FID $\downarrow$}  \\ 
% & &  & & \multicolumn{1}{c}{Food \citep{bossard2014food} }  & \multicolumn{1}{c}{Car \citep{gebru2017fine}}   & \multicolumn{1}{c}{Average} \\ \midrule
%     I  &  \ding{51} &    &  & 18.76 & 33.77 &  26.27 \\

    
%     % I  w/o ranking &  \ding{51} &    & & & 25.11 & 25.04 & -   \\ 
%     I-Sigmoid  &  \ding{51} &    &   & 20.61 & 38.43   & 29.52 \\ \midrule
%     II  &   & \ding{51}   &  & 53.47 & -   \\
%     III  &  \ding{51} & \ding{51}   &   & 19.76 & 27.80  & 23.78 \\   \midrule
%     % IV  &  \ding{51} &   & \ding{51}  & - & 18.45 & 43.80   & 31.13 \\           \midrule
%     IV  &  \ding{51} & \ding{51}    & \ding{51}  & \textbf{16.64} & \textbf{21.01}  & \textbf{18.83} \\
%     IV-layer  &  \ding{51} & \ding{51}    & \ding{51}    & 17.08 &  23.67  & 20.38 \\

% \bottomrule
%     \end{tabular}} 

%     \end{minipage}
    
% \end{table*}
\vspace{-3mm}
\subsection{Ablation Study}


% \documentclass{article}
% \usepackage[utf8]{inputenc}
% \usepackage{array} % 用于创建表格
% \usepackage{graphicx} % 用于wrapfig
% \usepackage{wrapfig} % 用于文字环绕

% \begin{document}

\begin{wrapfigure}{r}{0.6\textwidth} % 定义wrapfigure环境，r表示右侧环绕
  \centering % 居中表格
\begin{minipage}{1.0\linewidth}

     \caption{\textbf{Ablation studies based on DyDiT-S.} All models are trained in the cross-domain transfer learning manner. ``TDW'': Temporal-wise dynamic width. ``SDT'': Spatial-wise dynamic token. ``CMS'': Complete model self-distillation.} % ⭕️
          \label{tab:ablation_study}
  \centering
  \small
  %\resizebox{\linewidth}{!}{
\resizebox{1.0 \textwidth}{!}{    \begin{tabular}{c | c c c |c c c }
   \toprule 
    \multirow{2}{*}{Model} & \multirow{2}{*}{TDW} & \multirow{2}{*}{SDT} & \multirow{2}{*}{CMS}  & \multicolumn{3}{c}{FID $\downarrow$}  \\ 
& &  & & \multicolumn{1}{c}{Food}  & \multicolumn{1}{c}{Car}   & \multicolumn{1}{c}{Average} \\ \midrule
    I  &  \ding{51} &    &  & 18.76 & 33.77 &  26.27 \\

    
    % I  w/o ranking &  \ding{51} &    & & & 25.11 & 25.04 & -   \\ 
    I-Sigmoid  &  \ding{51} &    &   & 20.61 & 38.43   & 29.52 \\ \midrule
    II  &   & \ding{51}   &  & 53.47 & 66.20   & 59.84 \\
    III  &  \ding{51} & \ding{51}   &   & 19.76 & 27.80  & 23.78 \\   \midrule
    % IV  &  \ding{51} &   & \ding{51}  & - & 18.45 & 43.80   & 31.13 \\           \midrule
    IV  &  \ding{51} & \ding{51}    & \ding{51}  & \textbf{16.64} & \textbf{21.01}  & \textbf{18.83} \\
    IV-layer  &  \ding{51} & \ding{51}    & \ding{51}    & 17.08 &  23.67  & 20.38 \\

\bottomrule
    \end{tabular}} 
    \end{minipage}
     % \vspace{-3mm}
\end{wrapfigure}






% TODO 改成模块的名字
\vspace{-3mm}
\paragraph{Main Components.}
We first conduct experiments to verify the effectiveness of each component in our method. We summarize the results in Table~\ref{tab:ablation_study}. ``Model I''  and ``Model II''  denote  DiT with only the proposed temporal-wise dynamic width (TDW) and spatial-wise dynamic token (SDT), respectively. We can find that ``Model I'' performs much better than ``Model II''. The reason behind this lies in the fact that when the total FLOPs ratio $\lambda$ is set to 0.5, tokens in ``Model II'' have to skip most $\operatorname{MLP}$ blocks, leaving only $\operatorname{MHSA}$ blocks to process tokens, which hurts the performance significantly \citep{dong2021attention}. ``Model III'' represents the model that combines both TDW and SDT, achieving obviously better performance than ``Model I''  and ``Model II''. Given a computational budget, the combination of TDW and SDT allows the model to discover an optimal dynamic strategy from a broader architecture space, leading to improved performance. Finally, we introduce the proposed complete model self-distillation (CMS) to  ``Model II'', resulting in ``Model IV''. Its superior performance verifies the importance of maintaining a complete model during training.  % ⭕️


\vspace{-3mm}
\paragraph{Different designs in temporal-wise dynamic width.}
We further investigate an alternative approach in temporal-wise dynamic width. Instead of predicting the probability of top-$h$ heads/channels, the model directly estimates the probability of keeping and removing a head or channel at the current timestep using Gumbel-Softmax \citep{jang2016categorical}. This operation is similar to that adopted in dynamic token selection. However, this design does not capitalize on the prior knowledge of head/channel importance, necessitating the model to learn the significance of individual heads and channels from scratch. 
The results from the ``Model I-Sigmoid'' in Table~\ref{tab:ablation_study} also demonstrate that this alternative design leads to inferior performance.  % ⭕️




\paragraph{Effectiveness of fine-grained token skipping.}
We also explore an alternative design to conduct token selection in the SDT. Specifically, for each $\operatorname{MLP}$ block, a router determines whether all tokens should bypass the block or be processed by it. This modification causes the dynamic token selection mechanism to resemble a layer-skipping approach, similar to \citep{wang2018skipnet}. We replace the dynamic token selection in ``Model V'' with this design, resulting in ``Model V-Layer''.  As discussed in Section~\ref{sec:introduction}, different regions within an image may encounter varying challenges in estimating noise. The strategy of processing all tokens together does not adequately address this variability.   For instance, tokens from particularly challenging regions may have to skip certain blocks, leading to suboptimal noise prediction. The results presented in Table~\ref{tab:ablation_study} further confirm that the fine-grained token skipping, as employed by the spatial-wise dynamic method, significantly improves the performance of ``Model V'' compared to ``Model V-Layer''. % ⭕️

% skipping or processing all tokens together can not meet this requirement.
% This makes the dynamic token selection degrade to resemble a layer-skipping approach, similar to \citep{wang2018skipnet}. 

% For example, some tokens from those difficult regions have to skip some blocks, leading to unsatisfactory noise prediction. The results in Table~\ref{tab:ablation_study} also verify that the fine-grained token skipping in input-based dynamic token helps ``Model V'' surpass ``'Model V-Layer' obviously.



% First, we try to remove the importance score ranking from the ``Models I'', resulting in ``Model I w/o ranking''. In this model, all heads and channels keep the same with the original DiT.

% \begin{table}[t]
% \normalsize
% \addtolength{\tabcolsep}{0.5mm}
% \renewcommand{\arraystretch}{1.0}
%     \centering
%     \caption{\textbf{Albation Study.} ``TDW'': Time-based dynamic width. ``IDT'': Input-based dynamic token. ``CMD'': Complete model distillation.}
% \resizebox{0.8 \textwidth}{!}{    \begin{tabular}{c | c c c| c |c c c }
%     \toprule
%     \multirow{1}{*}{Model} & \multirow{1}{*}{TDW} & \multirow{1}{*}{IDT} & \multirow{1}{*}{CMD} & \multirow{1}{*}{FLOPs (G) $\downarrow$}  & \multicolumn{1}{c}{Food \citep{bossard2014food}}    & \multicolumn{1}{c}{Car \citep{gebru2017fine}}   & \multicolumn{1}{c}{Average}   \\ \midrule

%     I  &  \ding{51} &    &  & - & 18.76 & 33.77 &  26.27 \\
%     % I  w/o ranking &  \ding{51} &    & & & 25.11 & 25.04 & -   \\ 
%     I-Sigmoid  &  \ding{51} &    &  & - & 20.61 & 38.43   & 29.52 \\\midrule
%     II  &   & \ding{51}   & & - & 53.47 & -   \\
%     III  &  \ding{51} & \ding{51}   &  & - & 19.76 & 27.80  & 23.78 \\   \midrule
%     % IV  &  \ding{51} &   & \ding{51}  & - & 18.45 & 43.80   & 31.13 \\           \midrule
%     V  &  \ding{51} & \ding{51}    & \ding{51}  & - & \textbf{16.64} & \textbf{21.01}  & \textbf{18.83} \\
%     V-layer  &  \ding{51} & \ding{51}    & \ding{51}  &   & 17.08 &  23.67  & 20.38 \\

% \bottomrule
%     \end{tabular}} 
%     \label{tab:ablation_study}
% \end{table}





\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/visualization.pdf}

\caption{\textbf{Qualitative comparison of images generated by the DyDiT and DiT.} All models are of ``S'' size. Our method produces high-quality images and significantly enhances generation efficiency.
} 
 % ⭕️
 \vspace{-4mm}
\label{fig:visuzalization}
\end{figure*} 










% \begin{table}[t]
% \normalsize
% \addtolength{\tabcolsep}{0.5mm}
% \renewcommand{\arraystretch}{1.0}
%     \centering
%     \caption{\textbf{Scale up the size of DiT.} }
% \resizebox{0.8\textwidth}{!}{    \begin{tabular}{c | c | c | c| c}
%     \toprule
%     \multirow{1}{*}{Model} & \multirow{1}{*}{s/img $\downarrow$ } & \multirow{1}{*}{FLOPs (G) $\downarrow$}  & \multicolumn{1}{c}{FID $\downarrow$}   & \multicolumn{1}{c}{$\Delta$}  \\ \midrule

%     Original DiT-S  & 0.65  & 6.07   & 21.46 & - \\
%     DyDiT-S & 0.42 & 2.97 & 31.83  & +10.37 \\  \midrule

%     Original DiT-B  &   &    &  & - \\
%     DyDiT-B &  &  &   &  \\  \midrule

%     Original DiT-XL  &   &    &  & - \\
%     DyDiT-XL &  &  &   &  \\  \midrule
 

%     \end{tabular}}
%     \label{tab:sota_imagenet}
% \end{table}




% \paragraph{Effectiveness of self-distillation.}



% \paragraph{Effectiveness of uniform time-sampling.}



% \subsection{Experiments on Class-to-Image Generation}


% \paragraph{In-domain fine-tuning}








% \subsection{.}


% \subsection{Experiments on Text-to-Image Generation}











% We consider a more challenging scenario, where the model need to learn the dynamic str




\begin{table*}[!h]
\renewcommand{\arraystretch}{0.8}
% \vspace{-2mm}
      \begin{minipage}{0.49\linewidth}
        \centering
        \small
          \caption{\textbf{Combined with the efficient sampler.} Replacing
          250-step DDPM \citep{ho2020denoising} with 10-step DPM solver++ \citep{lu2022dpm} significantly enhances generation speed but also leads to a performance drop. In comparison to DiT-XL, the performance decline of DyDyT-XL is more modest. }
        %\resizebox{\linewidth}{!}{
\resizebox{1.0\textwidth}{!}{\begin{tabular}{c | c | c | c| c}
\toprule
    \multirow{1}{*}{Model}   & \multirow{1}{*}{Sampler}  & \multirow{1}{*}{s/img $\downarrow$ }  & \multicolumn{1}{c|}{FID $\downarrow$}   & \multicolumn{1}{c}{FID $\Delta \downarrow$ }  \\ \midrule

    DiT-XL    & 250-DDPM  & 10.22   & 2.27  & 0.00 \\
    DyDiT-XL  & 250-DDPM  & 6.47  & 2.14   & -0.13\\ \midrule


    DiT-XL    & 10-DPM solver++  & 0.45 & 11.66  & +9.39 \\
    DyDiT-XL  & 10-DPM solver++  & 0.29 & 11.21  & +8.94 \\ \bottomrule

    \end{tabular}}
        %}
   \label{tab:sampler}
    \end{minipage}
    \hfill %前后不要有空格
      \begin{minipage}{0.49\linewidth}
        \centering
        \small
        \caption{\textbf{Combined with DeepCache.} ``Interval'' denotes the interval of cached timestep in DeepCache \citep{ma2023deepcache}. ``FID $\Delta \downarrow$'' represents the FID discrepancy compared to DiT-XL with zero-interval.}   % ⭕️
     
\resizebox{1.0\textwidth}{!}{\begin{tabular}{c | c | c | c| c}
\toprule
    \multirow{1}{*}{Model}   & \multirow{1}{*}{Interval}  & \multirow{1}{*}{s/img $\downarrow$ }  & \multicolumn{1}{c|}{FID $\downarrow$}   & \multicolumn{1}{c}{FID $\Delta \downarrow$ }  \\ \midrule

    DiT-XL    & 0  & 10.22   & 2.27   & 0.00 \\ 
    DiT-XL    & 3  & 3.37    & 3.14   & +0.87 \\
    DiT-XL    & 8  & 1.45    & 21.42  & +19.15 \\ \midrule
    DyDiT-XL  & 0  & 6.47    & 2.14   & -0.13 \\ 
    DyDiT-XL  & 2  & 3.28    & 2.55   & +0.28 \\
    DyDiT-XL  & 5  &  1.34   & 9.07   & +6.80 \\ \bottomrule

    \end{tabular}}
        %}
\label{tab:cache}
    \end{minipage}
    \vspace{-5mm}
\end{table*}





\subsection{Compatibility with Efficient Diffusion Methods}
\vspace{-2mm}
% As a model-based approach to improve the generation efficiency, our method can be combined with other techniques, including efficient samplers and global acceleration approaches to further speed up the diffusion transformer. % ⭕️

% \vspace{-3mm}
\paragraph{Combined with efficient samplers.}
To demonstrate to compatibility with efficient samplers, we adopt DPM solver++ \citep{lu2022dpm} to reduce the sampling steps from 250 to just 10. This efficient sampler significantly accelerates the generation speed of both DiT-XL and DyDiT-XL. However, we observe that it also results in a performance drop. For instance, the FID score of our method increases to 7.23, which remains marginal compared to the drop observed in DiT-XL. This result indicates the potential of our approach when combined with efficient samplers, an promising direction in future research. % ⭕️
 
\vspace{-3mm}
\paragraph{Combined with global acceleration.}
DeepCache \citep{ma2023deepcache}, a train-free technique, is designed to globally accelerate the generation speed.  During generation, DeepCache caches featuremaps at specific timestep intervals and reusing these features across subsequent timesteps, thereby reducing generation time. We combine our approach with DeepCache. Results are presented in Table~\ref{tab:cache}. By cooperating with DeepCache, our model achieves further acceleration with only a marginal performance drop. When  DiT is integrated with DeepCache, it requires a longer interval to reach comparable speeds to our method, resulting in a inferior FID score. These results verify the compatibility and effectiveness of our approach in conjunction with DeepCache.  % ⭕️
 
% TODO 改成定性实验
\subsection{Qualitative comparison}
Figure~\ref{fig:visuzalization} illustrates the images generated by DyDiT-S on four fine-grained datasets, comparing them with those produced by the original DiT-S. Additionally, in Appendix~\ref{app:visualization}, we provide further examples of images generated by DyDiT-XL on the ImageNet dataset. These qualitative results validate that our method not only maintains the FID score but also produces realistic images. % ⭕️

% Notably, DyDiT-S achieves similar image quality to the original DiT while significantly reducing computational costs. 




